MAGELLAN: Metacognitive predictions of learning progress guide autotelic LLM agents in large goal spaces

Open-ended learning agents must efficiently prioritize goals in vast possibility spaces, focusing on those that maximize learning progress (LP). When such autotelic exploration is achieved by LLM agents trained with online RL in high-dimensional and evolving goal spaces, a key challenge for LP prediction is modeling one's own competence, a form of metacognitive monitoring. Traditional approaches either require extensive sampling or rely on brittle expert-defined goal groupings. We introduce MAGELLAN, a metacognitive framework that lets LLM agents learn to predict their competence and LP online. By capturing semantic relationships between goals, MAGELLAN enables sample-efficient LP estimation and dynamic adaptation to evolving goal spaces through generalization. In an interactive learning environment, we show that MAGELLAN improves LP prediction efficiency and goal prioritization, being the only method allowing the agent to fully master a large and evolving goal space. These results demonstrate how augmenting LLM agents with a metacognitive ability for LP predictions can effectively scale curriculum learning to open-ended goal spaces.

==> icml2025/intro_v3.tex <==

% opening example, language as universal goal space and the open-ended learning challenge
Imagine teaching a robot to ``grasp a glass", ``cook a risotto", or ``compose a poem." The space of possible goals we can express in language is effectively infinite, with tasks ranging from simple physical manipulations to complex creative endeavors. This richness of language makes it a powerful medium for specifying goals to artificial agents. However, it also poses a fundamental challenge: how can an agent efficiently explore and master an ever-expanding space of possible goals? This question lies at the heart of open-ended learning\,---\,the ability to continuously acquire new skills throughout one's lifetime.

% human open-ended learning, and the quest to model it computationally
Humans display a remarkable capacity for such open-ended learning, driven by a remarkable intrinsic motivation to imagine and pursue goals of our own making \citep{colas_autotelic_2022}. This autotelic learning ability allows us to progressively build increasingly complex skills, from an infant's first attempts to grasp objects to an adult mastering a musical instrument. Understanding and replicating this ability in artificial systems represents a fundamental challenge in AI, with implications for both advancing machine intelligence and illuminating human development \citep{schmidhuber_powerplay_2013, jiang2023general, Sigaud2023ADO}. 

% intrinsic motivations, focus on LP and how it explains human development and learning trajectories
Evolution appears to have equipped humans with sophisticated intrinsic motivations to tackle this challenge of navigating vast possibility spaces \citep{oudeyer2016evolution, gottlieb2018towards}. At the core of this ability is learning progress (LP)\,---\,the measurable improvement in one's ability to achieve goals \citep{kaplan2007progress}. Rather than randomly sampling from all possible goals or pursuing objectives that are too difficult, LP-driven learners focus on the ``Goldilocks zone" of activities where they are making the most progress \citep{kidd2015psychology}. This scaffolding effect of LP has been extensively documented in developmental psychology: infants systematically explore their environment by selecting activities of increasing difficulty \citep{oudeyer2016evolution}, while recent studies show that both children and adults explicitly track their learning progress to guide their choice of learning activities \cite{ten_humans_2021,leonard2023young}. 

% these ideas have been translated to AI, where LP has been used to train agents and let them organize their curricula
Inspired by these findings, researchers have worked to computationally model learning progress as a key mechanism for open-ended learning in artificial agents \citep{schmidhuber_possibility_1991, kaplan2007progress, baranes_active_2013}. By designing agents that aim to maximize their learning progress, researchers have created systems that effectively generate their own training curricula \citep{portelas_automatic_2020,romac_teachmyagent_2021}, leading to notable successes in both simulated and physical robotic tasks \citep{colas_curious_2019, portelas_teacher_2019, kanitscheider_multi-task_2021, forestier_intrinsically_2022}. 

% but existing methods are hard to scale when goal spaces becomes large
However, scaling these successes to true open-ended learning in vast language goal spaces introduces fundamental new challenges. Traditional approaches face a critical dilemma: they must either extensively sample each possible goal to directly measure competence (prohibitively expensive), or rely on predefined groupings of goals to share competence estimates (brittle and limiting). What we need instead is a way to leverage the semantic structure inherent in language itself\,---\,understanding that success at ``stacking red blocks" likely translates to ``stacking blue blocks" but only partially helps with ``building a pyramid".

% recent breakthroughs in LLM agents suggest a promising direction
Language-conditioned reinforcement learning (RL), and its most recent extension leveraging large language models (LLMs) allow to train agent policies that efficiently generalize across vast language goal spaces \cite{carta_grounding_2023, wen_entropy-regularized_2024, wen_reinforcing_2024}. Scaling LP estimations to these spaces requires comparable efforts at the \textit{metacognitive level}\,---\,\ie giving agents the ability to model their own competence and learn patterns in how skills generalize across related goals. This work proposes to develop such a capability. 

% magellan
We introduce \textbf{MAGELLAN} (\textbf{M}et\textbf{A}cognitive \textbf{GE}neralization of \textbf{L}earning progress in \textbf{LAN}guage model agents), a framework that enables LLM agents to learn to predict their own competence and learning progress online. The key insight of MAGELLAN is to leverage the LLM's semantic understanding: rather than treating each goal independently or relying on predefined groupings, MAGELLAN learns to map goals into a latent space where semantically similar goals naturally cluster together, allowing competence estimates to efficiently generalize across related goals. 

% experiments and contributions
To validate MAGELLAN, we conduct experiments in an interactive learning environment specifically designed to study commonsense-based generalization across a large space of language goals. Our results demonstrate that MAGELLAN:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=15pt]
    \item enables more accurate and sample-efficient learning progress estimation compared to traditional approaches,
    \item improves curriculum learning, allowing agents to master a large goal space where prior methods fail, 
    \item generalizes to predict competence on new goals, enabling rapid adaptation as the goal space evolves.   
\end{itemize}
Importantly, MAGELLAN achieves this without requiring any expert-defined goal groupings, learning to organize the goal space purely from experience. 

These results demonstrate how augmenting LLM agents with metacognitive abilities can effectively scale curriculum learning to open-ended goal spaces. Beyond our specific experiments, this work suggests that metacognition may be essential for truly open-ended learning systems, just as it appears to be in human learning. As we push towards more general artificial intelligence, the ability to model and predict one's own learning capabilities may become increasingly crucial.



==> icml2025/statement_V1.tex <==
% Following removed to gain space
% We start by defining learning progress for a policy $\pi$ w.r.t. a goal space $\mathcal{G}$. Considering that, at time $t$, $\pi$ has experienced and been updated on $t-1$ goals $\{g_1, g_2,...,g_{t-1}\} = \mathcal{E}_t$, we can define some competence measure $C_{\pi}(g|\mathcal{E}_t)$ for $\pi$ on some goal $g \in \mathcal{G}$ after having experienced $\mathcal{E}_t$. The expected learning progress of $\pi$ on $g$ at time $t$ is the competence change if $\pi$ experiences $g$: $LP_{\pi}(g) = C_{\pi}(g | \mathcal{E}_t \cup \{g\}) - C_{\pi}(g | \mathcal{E}_t)$. As future progress $C_{\pi}(g | \mathcal{E}_t)$ for all possible goals is usually unknown, most prior works approximate it using past progress between: $\hat{LP}_{\pi}(g) = C_{\pi}(g | \mathcal{E}_t) - C_{\pi}(g | \mathcal{E}_{t-1})$.




We start by defining learning progress for a policy $\pi$ w.r.t. a goal space $\mathcal{G}$ as the competence improvement on some goal $g$ when the policy practices $g$.
Here, we consider goals defined with natural language (i.e. $g \in \mathcal{G} \subset \mathcal{V}^K$ with $\mathcal{V}$ a vocabulary of possible tokens, $K$ the maximum number of tokens and $\mathcal{G}$ the set of goals) along with an LLM learner. We expect such an LLM-based policy to show generalization between semantically similar goals (i.e. competence transfer).

In experiments below, we focus on episodic RL with sparse and binary rewards (i.e. r=1 if the goal is reached, 0 otherwise). As the episode stops when a goal is reached or after a fixed number of steps, only two returns can be obtained for an episode where \( \pi \) tries to achieve the goal \( g \): 1 (success) or 0 (failure). We note an episode's outcome $\mathds{1}_{(\pi, g)}$. We thus define competence as the success probability: $\mathbb{P}_{\pi}(g) = \mathbb{E}_\pi\left[\mathds{1}_{(\pi, g)}\right]$. 

% When collecting multiple episodes of $\pi$ trying to achieve $g$, we define the success rate (SR) $SR_{\pi}(g)$ as the average outcome of these trials (i.e. a monte-carlo estimation of the success probability).

% We note these two possible returns $\mathds{1}_{(\pi, g)}$. In such settings, we define competence as the Success Rate (SR), denoted by:  

% \begin{equation}
%     SR_{\pi(g)} = \mathbb{E}_\pi\left[\mathds{1}_{(\pi, g)}\right].
% \end{equation}  


==> icml2025/statement_v2.tex <==
In this paper, we focus on episodic online goal-conditioned RL with sparse and binary rewards, defined on %. The aim is to train a policy $\pi$ on
a goal-augmented MDP $(S, A, P, G, R, S_0)$, with $S$ a set of states, $P$ the transition function of the environment, $A$ the action space, $G$ the goal space and $R:S\times G \rightarrow \{0;1\}$  a binary success function indicating whether a state $s \in S$ satisfies a goal $g \in G$. $S_0 \subseteq S$ stands as the set of initial states of the problem. The final aim is to discover the optimal policy $\pi^*$ that masters any goal in $G$ starting from any possible state in $S_0$. More specifically, we consider a textual environment where a prompting function $\phi:S\times G \rightarrow {\cal V}^K$ is given to transform any pair (state, goal) into a textual prompt of K tokens in a given vocabulary ${\cal V}$. % (with allows As we consider We define a task prompt  
Our aim is thus to maximize: 
$$J(\pi)=\mathbb{E}_{s_0 \sim {\cal U}(S_0), g \sim {\cal U}(G)} \left[\mathbb{P}_\pi(s_0,g) \right], $$
where $\cal U(\cal X)$ stands for the uniform distribution over a  set $X$ and $\mathbb{P}_\pi(s_0,g)$ is defined as the probability for $\pi$ starting from $s_0$ to achieve $g$ within an episode of $T$ steps: $\mathbb{P}_\pi(s_0,g) = \mathbb{E}_{\tau \sim \pi(\tau|s_0,g)}[\mathds{1}(\exists s_t \in \tau, R(s_t,g)=1)]$, with $\mathds{1}$ the indicator function. $\pi(\tau|s_0,g)$ is the distribution of episodes of $T$ steps,  starting from $s_0$ (i.e., $\tau=(s_0,a_0, % s_1, a_1, 
\ldots, a_{T-1}, s_T)$),  induced by policy $\pi$. $\pi$  selects any action $a_t \in A$ by sampling from a categorical distribution $\pi(.|\phi(s_t, g))$ at any step $t \in [[0,T-1]]$ of the episode.   


However, given the possibly huge number of $(s_0,g)$ combinations, the direct maximization of the problem as stated above may become particularly inefficient. %intractable.
Our aim is to leverage transfer of competences between problem configurations, and focus during training on tasks that maximize progress. In the following, we denote as $\pi^n$   %=\Xi(\pi^{n-1}, \Gamma^{n-1} \cup \{\tau^n\})$ % {\tau^i\}_{i \in [[1;N]])$ %$ \sim \pi(\tau|s_O,g))$
the policy obtained after $n$ episodes of an RL algorithm $\Xi$, using experience $\Gamma^{n}$ acquired from $n$ training episodes, where each episode $\tau^i$ from $\Gamma^{n}$ was obtained using $\pi^{i-1}$ on a training task sampled from a task selector %distribution 
$\eta({\cal T}^i|\pi^{i-1})$, with ${\cal T}^i \in \mathcal{E}_\mathcal{T} \equiv \{\phi(s,g)\}_{s \in S_0, g\in G}$ (i.e., $\mathcal{E}_\mathcal{T}$ is defined as the set of possible prompts for any combination of the starting configuration and goal to achieve). %  tasks  tuning on $n$ an initial policy on $\pi^{n-1}$ from experience $\Gamma^{n-1}$ at step $n-1$ augmented by a new episode sampled from $\pi^{n-1}$. % new experience acquired from sampling an episode from $$ 
Given a budget of N training episodes, we thus consider the problem of approaching the optimal selector $\eta^* = \arg\max_\eta J(\pi^N)$. We propose to build $\eta$ on a proxy of the learning progress (LP) at each training step $n$, where LP is defined for any task ${\cal T}=\phi(s_0,g)$ as the improvement of the policy at step $n$ after $k$ steps of RL tuning  $\Xi$ using %new experience acquired from
$k$ new episodes on task configuration $(s_0,g)$:  $LP^k_{\pi^n}({\cal T}=\phi(s_0,g))=\mathbb{P}_{\pi^{n+k}}(s_0,g) - \mathbb{P}_{\pi^{n}}(s_0,g)$. % training   %\sum_{n=1}^N \mathbb{E}_{\mathcal{T} \sim \eta(\pi^n)$$


%Next, we define the set of tasks of the problem as $\mathcal{E}_\mathcal{T}=\{\phi(s,g)\}_{s \in S_0, g\in G}$ the set of prompts for any combination of the starting configuration and goal to achieve. 

%face the aim is to within in a given number of N training episodes


 % (i.e. r=1 if the goal is reached, 0 otherwise).
%As the episode stops when a goal is reached or after a fixed number of steps, only two returns can be obtained for an episode where \( \pi \) tries to achieve the goal \( g \): 1 (success) or 0 (failure). We note an episode's outcome $\mathds{1}_{(\pi, g)}$. We thus define competence as the success probability: $\mathbb{P}_{\pi}(g) = \mathbb{E}_\pi\left[\mathds{1}_{(\pi, g)}\right]$.

==> previous_versions_introduction/new_intro.tex <==
Building open-ended learning agents has been a long-standing goal of research communities studying artificial agents \citep{schmidhuber_powerplay_2013, Sigaud2023ADO}. Yet, two major challenges remain: 1) creating and learning increasingly abstract goals and 2) navigating the possibly infinite space of possible goals \citep{jiang_learning_2023}. Several recent works tackled the first challenge by leveraging natural language as a compositional goal space that can be used to create new levels of abstractions \citep{wang_voyager_2023, colas_augmenting_2023, pourcel_aces_2024, colas_language_2020}. Notably, the use of LLM-based agents drastically impacted this choice, as such agents show efficient generalization capabilities when facing new goals. However, this also impacts the second challenge, as using natural language for the goal space creates an extremely wide space to navigate.

For this, the field of Automatic Curriculum Learning (ACL) \citep{portelas_automatic_2019} has gathered various methods to prioritize goals adapted to an online RL agent's competence. Among them, methods based on Learning Progress (LP) showed excellent capabilities on a broad range of tasks spanning from continuous control to complex tasks in Minecraft \citep{baranes_r-iac_2009, portelas_teacher_2019, kanitscheider_multi-task_2021}. Empowering these agents with an LP estimator also able to generalize over unseen goals would allow them to navigate spaces of natural language goals. However, current methods estimating the LP for natural language goals remain largely limited and cannot leverage the structure of language to generalize the LP to unseen goals.


% As such agents face increasingly complex tasks, properly ordering the learning curriculum has been shown as key \cite{jiang_learning_2023}. In this line, the field of Automatic Curriculum Learning (ACL) \citep{portelas_automatic_2019} has gathered various methods automatically designing a learning curriculum for RL agents. Among them, methods based on Learning Progress (LP) showed excellent capabilities on a broad range of tasks spanning from continuous control to complex tasks in Minecraft \citep{baranes_r-iac_2009, portelas_teacher_2019, kanitscheider_multi-task_2021}.

% However, measuring an agent’s current LP over large task spaces remains challenging as it requires a past and current evaluation of its competence on all tasks. Prior work approximates this LP by partitioning the task space and producing local estimations \citep{baranes_r-iac_2009, abdulhai_lmrl_2023}. % Nonetheless, obtaining meaningful partitions is not straightforward, and several prior studies leveraged natural language to obtain such a partition \citep{wang_voyager_2023, colas_augmenting_2023, pourcel_aces_2024}. 

% In addition to this, recent work also showed how natural language could be used to expand an agent’s current task space by imagining new goals \citep{colas_language_2020, colas_vygotskian_2022}. Leveraging language notably allows commonsense-based generalization of goals to create new ones. However, current methods estimating the LP cannot generalize to tasks unseen by the agent, limiting the possible use of LP to scaffold how the agent must learn new tasks.

% In particular, we consider the setup where an LLM-based RL agent, coupled with an LP-based ACL method ordering its curriculum, learns to solve tasks described with natural language. We equip the LLM agent with current and past competence estimators, which we train to match the agent’s competence over the task space. We then use these estimators to approximate the agent’s LP and leverage this estimation in our ACL teacher, allowing the LLM agent not only to increase its competence over a growing set of tasks but also to order its own curriculum. We call our method \textbf{M}et\textbf{A}cognitive \textbf{GE}neralization of \textbf{L}earning progress in \textbf{LAN}guage model agents (\textbf{MAGELLAN}).


In this paper, we study how an LLM-based agent learning with online RL could navigate a space of natural language goals using an LP estimator that generalizes. We introduce \textbf{M}et\textbf{A}cognitive \textbf{GE}neralization of \textbf{L}earning progress in \textbf{LAN}guage model agents: \textbf{MAGELLAN}. MAGELLAN leverages the LLM inside the agent to learn an LP estimator that can generalize. By augmenting the LLM-based RL agent with the metacognitive capacity of estimating its own competence and LP, MAGELLAN allows the agent to self-organize its curriculum to navigate the goal space. We evaluate MAGELLAN in the little-Zoo environment specifically designed as a carefully controlled experimental setup for commonsense-based generalization of agents in a textual environment. In particular, we study the following scientific questions:
\begin{itemize}
    \item \textbf{Q1.} Given an initial set of language goals, how does MAGELLAN enable the LLM-based online RL agent to estimate its own LP over these goals? How does it compare to more classic methods, which are precise but do not generalize?
    %How does MAGELLAN’s LP estimation compare to more classic methods, which are precise but do not generalize?
    \item \textbf{Q2.} Can MAGELLAN be used by the LLM agent to self-organize an efficient learning curriculum over these goals?
    \item \textbf{Q3.} How well can MAGELLAN predict the agent’s competence and LP on new unseen goals?
    \item \textbf{Q4.} When a set of new language goals are introduced, can MAGELLAN leverage its predictions of LP for these new goals to efficiently prioritize their exploration?
%When facing new tasks to learn, can MAGELLAN be used to prioritize tasks for its agent by generalizing its competence estimation?
\end{itemize}

We show that MAGELLAN not only approximates the LP efficiently but also adapts faster than standard LP estimation methods that need to evaluate the agent on a task to update their estimation. Equipped with MAGELLAN, our LLM-based RL agent successfully orders its curriculum of tasks. More importantly, it is able to estimate the agent's competence accurately on a test set of unseen tasks. Finally, we show this commonsense-based generalization of competence and LP can be used to design a curriculum for the agent when it faces new tasks to learn.



==> previous_versions_introduction/old_intro.tex <==
% LLM agents and Online RL, conclude on open-endedness+goal composition+large task spaces
Building open-ended learning agents has been a long-standing goal of research communities studying artificial agents \cite{schmidhuber_powerplay_2013}, intrinsic motivation \cite{} or continual learning \cite{}. The recent rise of Large Language Models (LLMs) has shifted the way these communities build agents. Equipped with commonsense knowledge and cultural priors of interestingness \cite{zhang_omni_2024,klissarov_motif_2023,du_guiding_2023}, LLMs are now being extensively used as agents that learn to solve goals in various interactive environments leveraging advanced prompting or Reinforcement Learning (RL) \citep{yao_react_2022,wang_jarvis-1_2023,wang_voyager_2023,abdulhai_lmrl_2023,carta_grounding_2023,wen_reinforcing_2024,zhai_fine-tuning_2024,zhou_archer_2024}. Prior work also showed such LLMs' abilities can be leverage to propose tasks to pursue \cite{wang_voyager_2023,colas_augmenting_2023,pourcel_aces_2024} when considering environments where a large amount of data exist on internet (and by extension in the LLMs' training dataset) on what humans usually achieve. Proposing tasks to achieved and properly scaffolding the agent's learning by organizing a curriculum of tasks to tackle has been shown as key \cite{jiang_learning_2023} when considering building open-ended learning agents in environments offering a large amount of possible tasks to achieve. 

% Scaffolding with Automatic Curriculum Learning => focus on LP method
Notably, the field of Automatic Curriculum Learning (ACL) \cite{portelas_automatic_2019} has gathered various methods automatically designing a learning curriculum for RL agents. Among these methods, Learning-Progress (LP) based methods were shown to be very efficient to drive the agent towards learning as many tasks as it can \cite{baranes_r-iac_2009,portelas_teacher_2019,kanitscheider_multi-task_2021}. They stem from the Learning Progress Hypothesis \cite{kaplan_search_2007}, stating that in some cases, animal and human learners are intrinsically motivated by activities on which they experience progress, that is, an improvement in a competence measure (e.g. prediction error \cite{schmidhuber_curious_1991} or return \cite{portelas_teacher_2019}). Measuring one's own LP has been shown to require advanced metacognition abilities as it involves accurately self-assessing and monitoring one's own competence \cite{abdelghani_guiding_2024,murayama_process_2019,ten_role_2022}.

% Challenges in self-evaluation of competence when considering the space of natural language goals
As highlighted by \citet{kaplan_search_2007}, measuring LP can be challenging, as naively estimating the learner's change of competence on a task involves the learner experiencing twice the exact same task. As a result, estimating the LP over very large task spaces can easily become intractable. While methods such as ALP-GMM \cite{portelas_teacher_2019} proposed solutions to approximate the LP over continuous task spaces, much remains to be done on discrete spaces. 

It is in particular the case with natural language, which has been recently shown as key for open-ended learning agents not only to partition the space of possible tasks but also to imagine and generate new goals \cite{colas_language_2020,colas_vygotskian_2022}. In addition to this, language also offers the clear advantage of being the key vector used by humans to transmit cultural aspects such as values, interestingness or commonsense. It nonetheless remains an open question if an LP estimator over natural language tasks could leverage these cultural aspects to generalize the LP to unseen tasks (e.g. if one knows the agent's competence on walking, it could infer that the agent's competence on running could be slightly worse). Designing such an estimator would greatly facilitate the computation of LP as one would not need the agent to see all the tasks but could rather rely on the generalization abilities of the estimator to infer which tasks the agent should be seeing next based on the tasks it has previously seen.

% Contributions
In this paper, we propose to tackle this generalizable LP estimation by training a model to approximate the LP by using an LLM backbone. When equipped with this new LP approximation, we first empirically study how an existing LP-based ACL method compares to its version using a more classic and precise LP estimation \cite{baranes_r-iac_2009} when scaffolding the curriculum of a simulated learner in an environment with textual tasks. We then equip an adaptation of an existing LLM-based RL agent \cite{carta_grounding_2023} with our new LP estimator and study how such an agent both learning a policy and self-assessing its performance to scaffold its own curriculum can be trained in a textual environment where estimating the LP over the possible textual tasks would benefit from commonsense abilities. We notably propose to analyze how the agents generalizes both its policy and competence estimation on task it has never experienced before. Finally, we go even further by studying how our agent can leverage its generalization abilities on both its policy and LP estimation when asked to learn various new set of goals. In particular, we analyze how the agent adapts when facing new goals similar to the ones it has experienced but also deceptive goals on which its commonsense knowledge may be wrong.

We summarize the scientific questions studied in our paper as follows:
\begin{itemize}
    \item \textbf{Q1.} Can we leverage an LLM to estimate an agent's competence and Learning Progress when the task space is natural language?
    \item \textbf{Q2.} How does a classic ACL method scaffolds a learner's curriculum on textual tasks when equipped with such an LP estimator?
    \item \textbf{Q3.} Can an LLM-based RL agent can at the same time 1) learn a policy with online RL, 2) self-assess and monitor its own competence and 3) scaffold its own curriculum, when equipped with our LP estimator?
    \item \textbf{Q4.} Do the commonsense knowledge of this LLM agent allows it to generalize its competence estimation to unseen goals and how does this estimation compares to its real performance (i.e. its policy's generalization abilities)?
    \item \textbf{Q5.} Can the agent leverage its generalizable LP estimation to scaffold its learning when facing new unseen goals, and how does this estimation adapt when facing deceptive tasks? 
\end{itemize}

We study these in a new set of environments (called the Zoo environments) specifically designed as a carefully controlled experimental setup for commonsense-based generalization of agents in a textual environment. We detail this environment in Section \ref{sec:zoo_env}, highlighting its key advantages and differences over prior work.
We show our LLM-based LP estimator efficiently approximates a learner's competence and results in a classic ACL method achieving similar performance when equipped with this approximation rather than a more precise but not generalizable LP estimator. We then show an LLM-based RL agent can successfully use this LP estimation to monitor and scaffold its own learning but also very efficiently approximate its own performance on new unseen tasks leveraging the commonsense abilities of the LLM backbone. Finally TODO: update with results on training on new goals.

To summarize, this work introduces and studies how an LLM agent can showcase metacognition abilities by not only learning how to solve tasks by interacting with online RL but also self-assess its own performance on tasks it is experiencing and leverage this ability to choose which tasks to train on. Additionally, we show such an agent is also capable of estimating its performance on tasks it has never seen and leverage this approximation to organize a curriculum when facing new tasks without even needing to evaluate its performance on them. Our in-depth analysis of such metacognition and generalization abilities in a carefully-designed and controlled experimental setup opens up for future work leveraging our agent's abilities in open-ended environments where the agent needs to generate its own goals and select which ones to pursue next.

TODO: Also open for future work leveraging the latent representation?
